DiffusionShield: A Watermark for Copyright Protection against Generative Diffusion Models

Recently, Generative Diffusion Models (GDMs) have showcased their remarkable capabilities in learning and generating images. A large community of GDMs has naturally emerged, further promoting the diversified applications of GDMs in various fields. However, this unrestricted proliferation has raised serious concerns about copyright protection. For example, artists including painters and photographers are becoming increasingly concerned that GDMs could effortlessly replicate their unique creative works without authorization. In response to these challenges, we introduce a novel watermarking scheme, DiffusionShield, tailored for GDMs. DiffusionShield protects images from copyright infringement by GDMs through encoding the ownership information into an imperceptible watermark and injecting it into the images. Its watermark can be easily learned by GDMs and will be reproduced in their generated images. By detecting the watermark from generated images, copyright infringement can be exposed with evidence. Benefiting from the uniformity of the watermarks and the joint optimization method, DiffusionShield ensures low distortion of the original image, high watermark detection performance, and the ability to embed lengthy messages. We conduct rigorous and comprehensive experiments to show the effectiveness of DiffusionShield in defending against infringement by GDMs and its superiority over traditional watermarking methods. The code for DiffusionShield is accessible in https://github.com/Yingqiancui/DiffusionShield.

==> secs/useless_expertiments.tex <==

% \section{Experiments}
% \label{sec:exp}

% \subsection{Setup}
% In our experiments, we use $8\times 8$ as the size of the basic blocks and encode the message into quarternary information, which means that totally we have 3 watermark patterns to be added to the different blocks of the images. For example, if the message we want to encode is `bird', we first transfer the characters into a binary message '01100010011010010111001001100100' based on the ASCII Table and then transfer the binary string into quarternary string '1202122113021210'. And we add the watermark pattern I, II, III to the corresponding blocks of the images. The experiments are conducted in three datasets, CIFAR10 at 32x32 resolution, CIFAR100 at 32x32 resolution, and STL10 at 64x64 resolution. Since the block size is $8\times8$, totally we need to divide the images of CIFAR10 and CIFAR100 into $4\times4$ blocks and divide the images of STL10 into $8\times8$ blocks. And we can inject 32 bits of information into the images of CIFAR10 and CIFAR100 and 128 bits into the images of STL10 dataset.

% We use the backbone of ResNet18 as the structure of the classifiers for identifying different watermark patterns. Since the size of the blocks is small, we remove the `conv4\_x' and `conv5\_x' layers and directly connect the average pooling layer to the `conv3\_x' layer in ResNet18. We use the SGD optimizer with momentum to be 0.9, learning rate to be 0.01 and weight decay to be $5\times 10^{-4}$. We consider different watermark budgets including 1/255, 2/255, 4/255 and 8/255. 

% We train the watermark patterns and the classifiers for recognizing the different patterns using the CIFAR10 dataset at 32x32 resolution. Because the watermark patterns can be universal across different datasets, the patterns generated with CIFAR10 are directly applied to watermark other datasets. The transferability of the watermark patterns across different datasets is demonstrated in Table 1, which shows the bit-wise accuracy of the classifier on different watermarked datasets with different watermarking budgets, where the watermark pattern is generated using only the CIFAR10 dataset.

% \begin{table}[h]
%   \caption{Bit-wise accuracy of the watermark decoder in initialized watermarked pattern and optimized watermark pattern (on CIFAR10).
% }
%   \label{tab:setting}
%   \centering
% %   \begin{threeparttable}

%   \begin{tabular}{ccccc}
%     \toprule
%     Budget & Initialized & Optimized \\
%     \midrule
%     \multirow{1}{*}{1/255} & 25.58\%  &	99.9850\%  \\ 
%     \multirow{1}{*}{2/255} & 36.41\% & 99.9988\% \\
%     \multirow{1}{*}{4/255} & 50.99\% & 100\% 	\\
%     \multirow{1}{*}{8/255} & 68.77\% & 100\% \\

%     \bottomrule
%   \end{tabular}

% \end{table}

% \begin{table}[h]
%   \caption{Bit-wise accuracy of the watermark decoder in training data
% }
%   \label{tab:setting}
%   \centering
% %   \begin{threeparttable}

%   \begin{tabular}{ccccc}
%     \toprule
%     Budget & CIFAR10 & CIFAR100 & STL10 & ImageNet20 \\
%     \midrule
%     \multirow{1}{*}{1/255} &  99.9850\% &	99.9850\% &	99.5931\% &	99.5246\%  \\ 
%     \multirow{1}{*}{2/255} & 99.9988\%	& 99.9981\%	&99.9284\% &	99.9243\% \\
%     \multirow{1}{*}{4/255} & 100\% &	100.0000\%	&99.9925\% & 99.9924\%\\
%     \multirow{1}{*}{8/255} & 100\% &	100.0000\%	&99.9988\% & 99.9998\% \\
%     \midrule
%     \multirow{1}{*}{DeepFake} &100\% &	99.9944\% &	99.9984\% &	99.9273\% \\
%     \bottomrule
%   \end{tabular}

% \end{table}



% We apply the improved DDPM training algorithm proposed by Nichol et. al (2021) to train the diffusion models on the data watermarked by our approach. We mainly considered two settings: the watermarked dataset is used to train the diffusion model separately, or together with other datasets which are not watermarked. In the second situation, we use the images of one randomly selected class of the dataset to represent the images owned by one copyright owner and consider the images of the other classes as datasets from other sources. In this case, only the images from the selected classes are watermarked. For example, for the CIFAR10 dataset, we select the bird class as the class to be protected and inject a watermark which embeds the quarternary string "1202122113021210" only to the bird images in the dataset. In the reference process, we apply the watermark decoding process to the images generated by the generative diffusion model to test whether the same watermark can be detected in the generated images.

% \subsection{Detect watermark from generative models trained on protected data}
% \jr{It seems freq and deepfake can not control budget.}

% \begin{table}[h]
%   \caption{Bit accuracy under different budgets on multiple datasets
% }
%   \label{tab:setting}
%   \centering
% %   \begin{threeparttable}

%   \begin{tabular}{ccccc}
%     \toprule
%     Budget & & CIFAR10 & CIFAR100 & STL10 \\
%     \midrule
%     \multirow{2}{*}{1/255} &  uncon.  &	96.0670\% &	 &  \\ & con. & 100\% & 68.8922\%  &  83.0320\%  \\ 
%     \multirow{2}{*}{2/255} &  uncon.  &	94.5139\% &	 &  \\ & con. & 100\% &75.2438\% & 99.8172\%   \\ 
%     \multirow{2}{*}{4/255} &  uncon.  & 94.4556\% &	100\% &   \\ & con. & 100\%   &  99.9906\% & 99.9875\% \\ 
%     \multirow{2}{*}{8/255} &  uncon.  &	100\% &	100\% &  \\ & con. & 100\% & 100\%  &  \\ 
%     \midrule

%     \multirow{2}{*}{Initialized} & uncon. &  &	 &  \\ & con. &  &  &  \\ 
%     \multirow{2}{*}{\jr{freq}} & uncon. & 0\%& 0\% &  0\%   \\
%     & con. & 0\% & 0\%  & 0\% \\ 
%     \multirow{2}{*}{deepfake} &  uncon. & 93.9740\% &	99.7725\% &  \\ &  con. & 100\% & 100\%  & 100\% \\ 
%     \bottomrule
%   \end{tabular}
% \end{table}




% \subsection{Encode different information for different copyright owner}

% \begin{table}[h]
%   \caption{Bit accuracy for different number of copyright owners \jr{conditional first}}
%   \label{tab:setting}
%   \centering
% %   \begin{threeparttable}

%   \begin{tabular}{ccccc}
%     \toprule
%     Dataset & Watermark & 1 & 4 & 10 \\
%     \midrule
%     \multirow{3}{*}{CIFAR-10} & (Initialized)  \\
%     & (freq)  \\
%     & (deepfake) &   99.9963\% & 99.9625\% & 99.9975\% \\
%     & Ours (2/255) & 100\% & 100\%  & 100\% \\
%     % \multirow{2}{*}{ImageNet-20} & (deepfake) \\
%     % & Ours \\
%     \bottomrule
%   \end{tabular}

% \end{table}



% \subsection{Encode more bits by different basic block}

% In some cases, the copyright owners may want to embed more message bits into the watermarks. In this section, we try to increase the capacity of the watermark by reducing the size of the basic blocks or turning the bit messages into octal string by using 7 watermark block patterns. Table 5 shows the capacity (the length of the encoded bit messages) of the watermark and the bit-wise accuracy of the decoding classifiers when using different settings in CIFAR-10 and STL-10. The budget of the watermark for both datasets is 4/255. The results demonstrates that our watermarking technique can still perform well when much more information is embedded in the watermark.



% \begin{table}[h]
%   \caption{Capacity and accuracy for different numbers of basic block classes and different block sizes}
%   \label{tab:setting}
%   \centering
% %   \begin{threeparttable}
    
%   \begin{tabular}{ccccccc}
%     \toprule
%  \multirow{2}{*}{Dataset} & \multirow{2}{*}{Size} & \multicolumn{2}{c}{capacity} & \multicolumn{2}{c}{bit accuracy} \\&&quant. & 
%  octal & quant.  &  octal  &   \\
%     \midrule
%     \multirow{2}{*}{CIFAR-10} &  $8\times8$   & 32 & 48 &100\% & 99.9958\%\\
%     & $4\times4$ &  128 & 192 & 99.9742\% & 99.9820\% \\
%     \multirow{2}{*}{STL-10} & $8\times8$ & 128 & 192\\
%     & $4\times4$ & 512 & 768\\
%     \bottomrule
%   \end{tabular}
% \end{table}




% \subsection{Robustness}

% Besides the demand for fidelity, We may also require the watermarks to be robust to image perturbations to ensure that the watermarks can still be detected if the generated images are subjected to post-processing or corruption in circulation. We consider five types of image corruption including gaussian noise, gaussian blur, random crop, grey scale transformation and jpeg compression, and conduct the corresponding augmentations respectively during the training of the watermark patterns to achieve robustness. 
% Table 6 shows the bit-wise accuracy of the detector on both clean and corrupted watermarked images generated by DDPM when different augmentations are applied. Since jpeg compression is not a differentiable process, we are not able to directly apply jpeg compression as an augmentation. But it is found that the watermark trained with gaussian noise augmentation is also robust to jpeg compression, so the results related to jpeg compression in Table 6 are the performance of the watermark trained with Gaussian noise augmentation when encountering jpeg compression. The results show that our watermarking technique is able to defend different corruptions if the corresponding augmentations are considered in the training process of the watermark patterns.

% \begin{table}[h]
%   \caption{Bit accuracy under different augmentation}
%   \label{tab:setting}
%   \centering
% %   \begin{threeparttable}

%   \begin{tabular}{cccc}
%     \toprule
%      &  & deepfake & ours \\
%     \midrule
%     \multirow{2}{*}{gaussian noise} & clean & 100\% & 100\%  \\
%     & robust & 74.5910\% & 98.1641\%\\
%     \midrule
%     \multirow{2}{*}{gaussian blur} & clean &100\% & 99.4094\%\\
%     & robust & 96.4770\% & 99.8484\%\\
%     \midrule
%     \multirow{2}{*}{crop} & clean& 100\% & 100\%\\
%     & robust &49.3830\% & 83.7891\%\\
%     \midrule
%     \multirow{2}{*}{greyscale} & clean  &100\% & 99.8313\% \\
%     & robust &51.4410\% & 99.8969\%\\
%     \midrule
%     \multirow{2}{*}{jpeg compression} & clean &100\% & 100\&\\
%     & robust &63.3450\% & 99.7625\%\\
    
%     \bottomrule
%   \end{tabular}

% \end{table}


% \subsubsection{Different accelerating sampling method when sampling}

% \begin{table}[h]
%   \caption{Bit accuracy under DDIM}
%   \label{tab:setting}
%   \centering
% %   \begin{threeparttable}

%   \begin{tabular}{cccc}
%     \toprule
%      & CIFAR10 & CIFAR100 & STL10  \\
%     \midrule
%     \multirow{1}{*}{ours 4/255}  &99.9953\% &99.9719\%\\
%     \multirow{1}{*}{deepfake} &99.9940\% &99.4825\% \\
%     % \multirow{3}{*}{ImageNet-20} & Image \\
%     % & (deepfake) \\
%     % & Ours \\
%     \bottomrule
%   \end{tabular}

% \end{table}


% \subsection{Fidelity}

% Partially added watermark.

% FID: watermark (training)

% FID: unwatermark - conditional (generated)

% \subsection{Fidelity}

% \begin{table}[h]
%   \caption{Fidelity}
%   \label{tab:setting}
%   \centering
% %   \begin{threeparttable}

%   \begin{tabular}{cccccc}
%     \toprule
%  & & CIFAR10 & CIFAR100 &  STL10 \\
%     \midrule
%     \multirow{5}{*}{Training} & Deepfake &
%     11.2863	& 45.6216 &	78.5507 \\ & ours 1/255 & 0.4076	&0.4412&	1.3729\\ & ours 2/255 & 2.3830	&2.6182	&4.7733\\ & ours 4/255 &6.6348 &	9.3292	&10.1295\\  & ours 8/255 & 11.2494 &10.6702&7.1974\\
%     \midrule
%  \multirow{4}{*}{Generated} & Deepfake 
%     & \\  & ours 2/255 &\\ & ours 4/255 &\\  & ours 8/255 &\\
%     \bottomrule
%   \end{tabular}

% \end{table}

